Dynamic Pricing and Learning with Long-term Reference Effects

We consider a dynamic pricing problem where customer response to the current price is impacted by the customer price expectation, aka reference price. We study a simple and novel reference price mechanism where reference price is the average of the past prices offered by the seller. As opposed to the more commonly studied exponential smoothing mechanism, in our reference price mechanism the prices offered by seller have a longer term effect on the future customer expectations. We show that under this mechanism, a markdown policy is near-optimal irrespective of the parameters of the model. This matches the common intuition that a seller may be better off by starting with a higher price and then decreasing it, as the customers feel like they are getting bargains on items that are ordinarily more expensive. For linear demand models, we also provide a detailed characterization of the near-optimal markdown policy along with an efficient way of computing it. We then consider a more challenging dynamic pricing and learning problem, where the demand model parameters are apriori unknown, and the seller needs to learn them online from the customers' responses to the offered prices while simultaneously optimizing revenue. The objective is to minimize regret, i.e., the $T$-round revenue loss compared to a clairvoyant optimal policy. This task essentially amounts to learning a non-stationary optimal policy in a time-variant Markov Decision Process (MDP). For linear demand models, we provide an efficient learning algorithm with an optimal $\tilde{O}(\sqrt{T})$ regret upper bound.

==> algo-design/6-algo-arbitrary-ref-new.tex <==


\newcommand{\conGreedyPrice}{p^{\cc{CGR}}}


In this section, we show that how to generalize \Cref{algo:equal ref}
to solve the case when the customers have arbitrary reference effects $(\positiveRef, \negativeRef)$. 
Recall that in \Cref{prop:approx markdown structure t_1}, 
we show for any $(\positiveRef, \negativeRef)$, there exists a 
markdown price curve $\approxMD(\priceUB, t_1, \truePara)$ 
with the policy parameter $\truePara = (\trueCOne, \trueCTwo)$
can achieve nearly optimal payoff for any starting time.
Moreover, such policy parameter $\truePara = (\trueCOne, \trueCTwo)$ with $\trueCOne = \frac{\positiveRef}{2(\baseDemandParaA + \positiveRef)}, \trueCTwo = \frac{\baseDemandParaB}{2(\baseDemandParaA + \positiveRef)}$ actually does not depend on the negative reference effect $\negativeRef$. 
Thus, similar to \Cref{algo:equal ref} for $\positiveRef = \negativeRef$,
it suffices to learn the policy parameter $\truePara$. 
In below, we detail main changes to generalize \Cref{algo:equal ref} for arbitrary
$(\positiveRef, \negativeRef)$:
\squishlist
    \item \textbf{Careful choices of reference prices $\{\firstRePrice, \secondRePrice\}$ in \expPhaseOne\ and {\color{blue}{\cc{2}}}}:
    When $\positiveRef = \negativeRef$, 
    in the exploration phase of \Cref{algo:equal ref}, 
    we learn two estimates of the greedy prices to learn the true policy parameter $\truePara$, 
    leveraging the relation between the greedy price and $\truePara$
    given by \eqref{eq:compute greedy}.
    However, when we have $\positiveRef \neq \negativeRef$, the greedy price 
    $\greedyPrice(\rePrice)$ may not equal to $\trueCOne \rePrice + \trueCTwo$.
    Moreover, the single-shot revenue function $\staticRev{\cdot, \rePrice}$ may not be 
    concave due to $\positiveRef \neq \negativeRef$.
    To fix this issue, 
    % fix any reference price $\rePrice\in[0, \priceUB]$,
    we carefully choose the reference prices that are used to learn the corresponding greedy prices. In particular, 
    we choose a reference price $\rePrice$ in a way such that 
    the single-shot revenue function $\staticRev{\cdot, \rePrice}$ has a maximizer
    strictly in $(0, \rePrice)$ and we show that such reference always exists (see \Cref{lem:constrained greedy}).
    In doing so, we can ensure that during the exploration phase, one only needs 
    to query the price in the range $(0, \rePrice)$ (this can be achieved 
    by change the projection interval to be $(\distance, \rePrice-\distance)$ in 
    \Cref{algo:zeroth-order arbitrary}), and 
    the single-shot revenue function $\staticRev{\cdot, \rePrice}$ is guaranteed to 
    be concave over the range $(0, \rePrice)$, i.e., 
    $\staticRev{p, \rePrice} = p\left(\baseDemand(p) + \positiveRef(\rePrice-p)\right)$
    for any $p\in(0, \rePrice)$.
    In doing so, the relation between the greedy prices and the true policy 
    parameter still holds as in \eqref{eq:compute greedy}.
    Thus, we are still be able to learn two greedy prices 
    to compute an estimate for the true policy parameter $\truePara$.
    
    \item \textbf{Compute and implement $\approxMD(\priceUB, \exploitT, \paraEst)$ in \exploitPhase}:
    Unlike using price curve 
    $\approxMD(\rePrice_{\exploitT}, \exploitT, \paraEst)$
    in \exploitPhase\ for $\positiveRef=\negativeRef$, 
    here, we compute the price curve $\approxMD(\priceUB, \exploitT, \paraEst)$
    using the starting reference price $\priceUB$.
\squishend



















==> algo-design/apx-generalized-linear.tex <==



\newcommand{\linkFn}{h}
\newcommand{\approxPolicy}{\bar{\pi}}


We consider generalized linear model
where $\baseDemand(p; \baseDemandParaA, \baseDemandParaB)
= \linkFn(\baseDemandParaB -\baseDemandParaA p)$
where $\linkFn(\cdot): \R\rightarrow \R$ is a link function. 
Let $\negativeRef = \positiveRef = \eta$.
Fix a reference price $\rePrice\in[0, \priceUB]$, we have
\begin{align*}
    \linkFn(\baseDemandParaB - \baseDemandParaA \greedyPrice(\rePrice)) - \baseDemandParaA \greedyPrice(\rePrice) \linkFn'(\baseDemandParaB - \baseDemandParaA \greedyPrice(\rePrice))
    + \eta \rePrice - 2\eta \greedyPrice(\rePrice) = 0
\end{align*}
Let $q^{\cc{GR}} (\rePrice)\triangleq \baseDemandParaB - \baseDemandParaA \greedyPrice(\rePrice)$, 
we then have
\begin{align*}
    \linkFn(q^{\cc{GR}}(\rePrice)) - (\baseDemandParaB - q^{\cc{GR}}(\rePrice)) \linkFn'(q^{\cc{GR}}(\rePrice))
    + \eta \rePrice - 2\eta\frac{\baseDemandParaB - q^{\cc{GR}}(\rePrice)}{\baseDemandParaA} = 0
\end{align*}
Fix a time window $[t_1, t_2]$,
by first-order condition, we also have
\begin{align*}
    \linkFn(\baseDemandParaB - \baseDemandParaA p_t) - \baseDemandParaA p_t \linkFn'(\baseDemandParaB - \baseDemandParaA p_t) - 2\eta p_t + \eta\left(\rePrice_t + \sum_{s=t+1}^{t_2} \frac{p_s}{s}\right) & = 0\\
    \linkFn(\baseDemandParaB - \baseDemandParaA p_{t+1}) - \baseDemandParaA p_{t+1} \linkFn'(\baseDemandParaB - \baseDemandParaA p_{t+1}) - 2\eta p_{t+1} + \eta\left(\rePrice_{t+1} + \sum_{s=t+2}^{t_2} \frac{p_s}{s}\right)
    & = 0
\end{align*}
Thus, we have
\begin{align*}
    \linkFn(\baseDemandParaB - \baseDemandParaA p_t) 
    -\baseDemandParaA p_t \linkFn'(\baseDemandParaB - \baseDemandParaA p_t)
    - \left(\linkFn(\baseDemandParaB - \baseDemandParaA p_{t+1}) 
    - \baseDemandParaA p_{t+1} \linkFn'(\baseDemandParaB - \baseDemandParaA p_{t+1}) \right) = (p_t - p_{t+1}) \left(2\eta + \frac{\eta}{t+1}\right) - \frac{\eta\rePrice_t}{t+1}
\end{align*}
Let $q_t \triangleq \baseDemandParaB - \baseDemandParaA p_t, 
q_{t+1}\triangleq \baseDemandParaB - \baseDemandParaA q_{t+1}$, we have
\begin{align*}
    \linkFn(q_t) 
    -(\baseDemandParaB-q_t)\linkFn'(q_t)
    - \left(\linkFn(q_{t+1}) 
    -  (\baseDemandParaB-q_{t+1}) \linkFn'(q_{t+1}) \right) = \frac{q_{t+1} -q_t}{\baseDemandParaA} \left(2\eta + \frac{\eta}{t+1}\right) - \frac{\eta\rePrice_t}{t+1}
\end{align*}
Rearranging the above terms, we have
\begin{align*}
    \frac{\linkFn(q_t) - \linkFn(q_{t+1}) + q_t \linkFn'(q_t) - q_{t+1} \linkFn'(q_{t+1})}{\linkFn'(q_t) - \linkFn'(q_{t+1})} = \baseDemandParaB +  
\end{align*}

For a generalized linear demand with link function $\linkFn(\cdot)$,
by first-order condition, the optimal pricing policy 
$\pvec^* = (p^*_t)_{t\in[t_1, t_2]}$ must satisfy that
\begin{align}
    2\eta p_t^* - \eta \frac{t_1\rePrice_{t_1} + p_{t_1}^*+\ldots +p_{t-1}^*}{t} - \eta \sum_{s=t+1}^{t_2} \frac{p_s^*}{s} 
    % & = \baseDemand(p_t^*) + p_t^* \baseDemand'(p_t^*) \\
    & = \linkFn(\baseDemandParaB - \baseDemandParaA p_t^*)
    - \baseDemandParaA p_t^* \linkFn'(\baseDemandParaB - \baseDemandParaA p_t^*)
\end{align}
Rearranging terms we have
\begin{align}
    {\color{red} 2\eta p_t^* - \eta \frac{p_{t_1}^*+\ldots +p_{t-1}^*}{t}
    - \eta \sum_{s=t+1}^{t_2} \frac{p_s^*}{s} 
    - \linkFn(\baseDemandParaB - \baseDemandParaA p_t^*)
    + \baseDemandParaA p_t^* \linkFn'(\baseDemandParaB - \baseDemandParaA p_t^*)
    = \eta\frac{t_1\rePrice_{t_1}}{t}}
\end{align}
When link function $h(x) = x$, we have 
\begin{align}
    2\eta p_t^* - \eta \frac{p_{t_1}^*+\ldots +p_{t-1}^*}{t}
    - \eta \sum_{s=t+1}^{t_2} \frac{p_s^*}{s} 
    - \baseDemandParaB + 2\baseDemandParaA p_t^*
    & = \eta\frac{t_1\rePrice_{t_1}}{t} \\
    \Leftrightarrow ~ 
    p_t^* - C_1^* \frac{p_{t_1}^*+\ldots +p_{t-1}^*}{t}
    - 
    C_1^* \sum_{s=t+1}^{t_2} \frac{p_s^*}{s} 
    & = C_2^* + C_1^* \frac{t_1\rePrice_{t_1}}{t}
\end{align}
where $C_1^* = \frac{\eta}{2(\baseDemandParaA+\eta)}, 
C_2^* = \frac{\baseDemandParaB}{2(\baseDemandParaA+\eta)}$.

where $\rePrice_t^* = \sfrac{(t_1\rePrice + \sum_{s=t_1}^{t-1} p_s^*)}{t}$. 
Let $q_t^* = \baseDemandParaB - \baseDemandParaA p_t^*$ for all 
$t\in[t_1, t_2]$, we then have
\begin{align*}
    2\eta \frac{\baseDemandParaB - q_t^*}{\baseDemandParaA}
    - \eta \rePrice_t^* - \eta \sum_{s=t+1}^{t_2 }\frac{\baseDemandParaB - p_s^*}{\baseDemandParaA s}
    = \linkFn(q_t^*) - (\baseDemandParaB - q_t^*) \linkFn'(q_t^*)
\end{align*}

\newpage 
\wt{valuation function is monotone with respect to the state $\rePrice$, tradeoff between greedy price and future price}

Let the single-round revenue function be 
$R(p; \rePrice) = p \baseDemand(p) + p \eta (\rePrice - p)$.
We define the following valuation function 
\begin{align}
    \label{eq:valuation fn}
    V(\rePrice, t) \triangleq \max_{p\in[\priceLB, \priceUB]}
    Q\left(p; \rePrice, t\right)
    = 
    \max_{p\in[\priceLB, \priceUB]}
    R(p; \rePrice) + V\left(\frac{t\rePrice + p}{t+1}, t+1\right)
\end{align}
We denote partial derivatives by using subscripts. 
A star superscript denotes the optimum.
By first-order condition, we know that the optimal price $p_t^*$ 
must satisfy
\begin{align}
    \label{eq:foc}
    R_p(p_t^*; \rePrice) + V_r\left(\frac{t\rePrice + p_t^*}{t+1}, t+1\right) \frac{1}{t+1} = 0
\end{align}
By envelope theorem, we have
\begin{align}
    \label{eq:envelope}
    V_r(\rePrice, t) = 
    R_r(p_t^*; \rePrice) + V_r\left(\frac{t\rePrice + p_t^*}{t+1}, t+1\right) \frac{t}{t+1}
\end{align}
From \eqref{eq:foc}, we have 
$V_r\left(\frac{t\rePrice + p_t^*}{t+1}, t+1\right) = -(t+1) R_p(p_t^*; \rePrice)$,
substituting it in \eqref{eq:envelope} and we get
\begin{align}
    V_r(\rePrice, t) 
    & = 
    R_r(p_t^*; \rePrice) -t R_p(p_t^*; \rePrice) 
    = \eta p_t^*  - t\left(p_t^*\baseDemand'(p_t^*) + \baseDemand(p_t^*) + \eta \rePrice -2\eta p_t^*\right)
    % & = -t \eta
\end{align}
Thus, we can also deduce that 
\begin{align}
    V_r\left(\frac{t\rePrice + p_t^*}{t+1}, t+1\right) = 
    R_r\left(p_{t+1}^*;\frac{t\rePrice + p_t^*}{t+1}\right) - (t+1) R_p\left(p_{t+1}^*; \frac{t\rePrice + p_t^*}{t+1}\right)
\end{align}
\wt{
\begin{align*}
    V_{p}\left(\frac{t\rePrice + p}{t+1}, t+1\right)
    & = \frac{1}{t+1} V_r\left(\frac{t\rePrice + p}{t+1}, t+1\right)\\
    & = 
    \frac{1}{t+1}  
    \left(R_r\left(p^*\left(\frac{t\rePrice + p}{t+1}\right); \frac{t\rePrice + p}{t+1}\right) - (t+1) R_{p}\left(p^*\left(\frac{t\rePrice + p}{t+1}\right); \frac{t\rePrice + p}{t+1}\right) 
    \right) \\
    & = 
    \frac{1}{t+1}  
    \left(\eta p^*\left(\frac{t\rePrice + p}{t+1}\right) - (t+1) R_{p}\left(p^*\left(\frac{t\rePrice + p}{t+1}\right); \frac{t\rePrice + p}{t+1}\right) 
    \right)\\ 
    & =  \frac{\eta p^*\left(\frac{t\rePrice + p}{t+1}\right)}{t+1}
    - R_{p}\left(p^*\left(\frac{t\rePrice + p}{t+1}\right); \frac{t\rePrice + p}{t+1}\right)  \ge 0
\end{align*}
where $p^*\left(\frac{t\rePrice + p}{t+1}\right) \triangleq \argmax_{p\in[\priceLB, \priceUB]} Q\left(p; \frac{t\rePrice + p}{t+1}, t+1\right)$
}
Finally, substitute the above formula into \eqref{eq:foc} and obtain a condition which does not depend on the value function anymore:
\begin{align}
    & {\color{red} R_p(p_t^*; \rePrice) + 
    \frac{1}{t+1}R_r\left(p_{t+1}^*;\frac{t\rePrice + p_t^*}{t+1}\right) - R_p\left(p_{t+1}^*; \frac{t\rePrice + p_t^*}{t+1}\right) = 0 } \\
    \Leftrightarrow ~ 
    & {\color{red} R_p(p_t^*; \rePrice) + 
    \frac{1}{t+1}\eta p_{t+1}^* - R_p\left(p_{t+1}^*; \frac{t\rePrice + p_t^*}{t+1}\right) = 0} \\
    % \Leftrightarrow ~ 
    % & p_t^* \baseDemand'(p_t^*) + \baseDemand(p_t^*) +\eta \rePrice - 2\eta p_t^*  
    % + \frac{1}{t+1}\eta p_{t+1}^* 
    % - \left(p_{t+1}^* \baseDemand'(p_{t+1}^*) + \baseDemand(p_{t+1}^*) +\eta \frac{t\rePrice + p_t^*}{t+1} - 2\eta p_{t+1}^*\right) = 0 \\
    % \Leftrightarrow ~ 
    % & p_t^* \baseDemand'(p_t^*) + \baseDemand(p_t^*) 
    % - \left(p_{t+1}^* \baseDemand'(p_{t+1}^*) + \baseDemand(p_{t+1}^*) \right) = 
    % \left(2\eta + \frac{\eta}{t+1}\right) (p_t^*   - p_{t+1}^*)
    % - \frac{\eta }{t+1} \rePrice\\
    \Rightarrow ~ 
    & R_p\left(p_t^*;\rePrice\right)
    = -\eta \sum_{s=t+1}^T \frac{p_s^*}{s}
\end{align}

\wt{how does $V(\rePrice, t) - V(\rePrice_{t+1}, t+1)$ change $p_t, p_{t+1}$ such that }
\begin{align*}
    {\color{red} R_p(p_t; \rePrice) + 
    \frac{1}{t+1}\eta p_{t+1} - R_p\left(p_{t+1}; \frac{t\rePrice + p_t}{t+1}\right) = \varepsilon t}
\end{align*}
% \wt{$Q(p, \rePrice, t)$}
where we have used the fact that $R_\rePrice(p;\rePrice) = \eta p$, 
and $R_p(p;\rePrice) = p\baseDemand'(p) + \baseDemand(p) + \eta \rePrice -2\eta p$.

We have 
\begin{align*}
    R_p\left(\pi^*(\rePrice, t); \rePrice\right)
    + \frac{\eta}{t+1} \pi^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right)
    - 
    R_p\left(\pi^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right); \frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}\right) = 0
\end{align*}
Use $R_p(\pi^*(\rePrice, t)) \approx R''(\greedyPrice(\rePrice)) (\pi^*(\rePrice, t) - \greedyPrice(\rePrice))$,
we have
\begin{align*}
    \pi^*(\rePrice, t) = & \greedyPrice(\rePrice) - \frac{1}{R''(\greedyPrice(\rePrice))}
    \left(\frac{\eta}{t+1} \pi^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right)\right. \\
    - &  
    \left.R''\left(\greedyPrice\left(\pi^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right)\right)\right) \left(\pi^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right) - \greedyPrice\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}\right)\right)
    \right)
\end{align*}

Thus, we have
\begin{align*}
    \pi^*(\rePrice, T) 
    & = \greedyPrice(\rePrice);\\
    \pi^*(\rePrice, T-1) 
    & \approx 
    \greedyPrice(\rePrice) 
    - \frac{\eta }{ R''(\greedyPrice(\rePrice))}\cdot \frac{\pi^*\left(\frac{(T-1)\rePrice + \pi^*(\rePrice, T-1)}{T}, T\right)}{T} \\
    &\le  
    \greedyPrice(\rePrice) 
    - \frac{\eta }{ R''(\greedyPrice(\rePrice))}\cdot \frac{\pi^*\left(\frac{(T-1)\rePrice + \priceUB }{T}, T\right)}{T}  \\
    \pi^*(\rePrice, T-2) 
    & \approx  
    \greedyPrice(\rePrice) 
    - \frac{\eta  }{R''(\greedyPrice(\rePrice))} \cdot \left(\frac{\pi^*(\rePrice_T^*, T)}{T} + \frac{\pi^*(\rePrice_{T-1}^*, T-1)}{T-1}\right)\\
    & = \greedyPrice(\rePrice) 
    - \frac{\eta  }{R''(\greedyPrice(\rePrice))} \cdot \left(\frac{\pi^*\left(\frac{(T-2)\rePrice + \pi^*(\rePrice, T-2) + \pi^*(\rePrice_{T-1}^*, T-1) }{T}, T\right)}{T} + \frac{\pi^*\left(\frac{(T-2)\rePrice + \pi^*(\rePrice, T-2) }{T-1}, T-1\right)}{T-1}\right) 
    \\
    \pi^*(\rePrice, t) 
    & \approx  \greedyPrice(\rePrice) 
    - \frac{\eta  }{R''(\greedyPrice(\rePrice))} \cdot
    \sum_{s=t+1}^T \frac{\pi^*(\rePrice_s^*, s)}{s}
\end{align*}

% Use $R_p(p_t^*) \approx R''(\greedyPrice(\rePrice)) (p_t^* - \greedyPrice(\rePrice))$,
% we have
% \begin{align*}
%     p_T^* 
%     & = \greedyPrice(\rePrice) \\
%     p_{T-1}^* 
%     & \approx 
%     \greedyPrice(\rePrice_{T-1}) 
%     - \frac{\eta  }{ R''(\greedyPrice(\rePrice_{T-1}))}\cdot \frac{p_T^*}{T} \\
%     & = \greedyPrice(\rePrice_{T-1}) 
%     - \frac{\eta  }{ R''(\greedyPrice(\rePrice_{T-1}))}\cdot \frac{\greedyPrice\left(\frac{(T-1)\rePrice_{T-1} + p_{T-1}^*}{T}\right)}{T}\\
%     p_{T-2}^* 
%     & \approx \greedyPrice(\rePrice_{T-2}) 
%     - \frac{\eta  }{R''(\greedyPrice(\rePrice_{T-2}))} \cdot\left(\frac{p_T^*}{T} + \frac{p_{T-1}^*}{T-1}\right)\\
%     & \vdots\\
%     p_{t}^* 
%     & \approx \greedyPrice(\rePrice_{t}) 
%     - \frac{\eta  }{R''(\greedyPrice(\rePrice_{t}))} \cdot \sum_{s=t+1}^T \frac{p_s^*}{s}
% \end{align*}

If we plug in $\baseDemand(p) = \baseDemandParaB -\baseDemandParaA p$,
the above equality gives us 
\begin{align}
    \label{linear opt}
    \pi^*(\rePrice, t)
    = \pi^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1 \right) + 
    \frac{\trueCOne \rePrice}{t+1 +\trueCOne}
\end{align}
where $\trueCOne = \frac{\eta}{2(\baseDemandParaA+\eta)}$.

\begin{lemma}
For any $t\in[T]$, we have 
\begin{align*}
    0\le \pi_{\rePrice}^*(\rePrice, t) \le 
    \frac{\trueCOne }{T+1-t}
\end{align*}
\end{lemma}
\begin{proof}
We prove by induction. 
When $t = T$, we know that 
\begin{align*}
    \pi^*(\rePrice, T) = \greedyPrice(\rePrice)
    = \trueCOne \rePrice + \trueCTwo
\end{align*}
Thus, we have $\pi_{\rePrice}^*(\rePrice, T) = \trueCOne$. 
Suppose that we have at time $t+1$, we have
\begin{align*}
    0 \le \pi_{\rePrice}^*(\rePrice, t+1) \le 
    \frac{\trueCOne }{T-t}
\end{align*}
Taking derivatives w.r.t to the reference price on both sides of \eqref{linear opt}, we then have
\begin{align*}
    \pi_{\rePrice}^*(\rePrice, t)
    & = 
    \pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1 \right)\cdot 
    \frac{t + \pi_{\rePrice}^*(\rePrice, t)}{t+1} 
     + 
    \frac{\trueCOne}{t+1 +\trueCOne} \\
    \Rightarrow ~ 
    \pi_{\rePrice}^*(\rePrice, t) & = 
    \frac{\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right) \frac{t}{t+1} + \frac{\trueCOne}{t+1 +\trueCOne}}{1 - \frac{1}{t+1}\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}\right)}
\end{align*}
Clearly, we also have $\pi_{\rePrice}^*(\rePrice, t)\ge 0$ as we have $1 - \frac{1}{t+1}\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}\right) 
\ge 1- \frac{1}{t+1}\frac{\trueCOne}{T-t} > 0$. 
Now to prove 
$\pi_{\rePrice}^*(\rePrice, t) \le \frac{\trueCOne}{T+1 - t}$, it suffices to prove 
\begin{align}
    \label{ineq:helper opt derivative}
    \frac{\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right) \frac{t}{t+1} + \frac{\trueCOne}{t+1 +\trueCOne}}{1 - \frac{1}{t+1}\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}\right)} 
    \le 
    \frac{\trueCOne}{T+1 - t}
\end{align}
Notice that by induction hypothesis, LHS of \eqref{ineq:helper opt derivative} satisfies:
\begin{align*}
    \frac{\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}, t+1\right) \frac{t}{t+1} + \frac{\trueCOne}{t+1 +\trueCOne}}{1 - \frac{1}{t+1}\pi_{\rePrice}^*\left(\frac{t\rePrice + \pi^*(\rePrice, t)}{t+1}\right)} 
    \le \frac{\frac{t}{t+1} \frac{\trueCOne}{T-t} + \frac{\trueCOne}{t+1 +\trueCOne}}{1 - \frac{1}{t+1}\frac{\trueCOne}{T - t}}
\end{align*}
Thus, it suffices to show 
\begin{align*}
    \frac{\frac{t}{t+1} \frac{\trueCOne}{T-t} + \frac{\trueCOne}{t+1 +\trueCOne}}{1 - \frac{1}{t+1}\frac{\trueCOne}{T - t}}
    \le 
    \frac{\trueCOne }{T+1 - t}
\end{align*}
It is easy to see that the function 
$f(t) = \frac{\frac{t}{t+1} \frac{1}{T-t} + \frac{1}{t+1 +\trueCOne}}{1 - \frac{\trueCOne}{T - t}} - \frac{1}{T+1 - t}$
\end{proof}

\begin{definition}
Consider following pricing policy: 
\begin{align*}
    \approxPolicy(\rePrice, t) = 
    \greedyPrice(\rePrice) 
    - \frac{\eta  }{R''(\greedyPrice(\rePrice))} \cdot
    \sum_{s=t+1}^T \frac{\pi^*\left(\frac{t\rePrice + (s-t)\priceUB}{s}, s\right)}{s}
\end{align*}
\end{definition}



\wt{The analysis here not finish ...}




==> algo-design/apx-proof-arbitrary-ref.tex <==

The modified algorithm for \Cref{algo:zeroth-order} for $\positiveRef\neq\negativeRef$
is provided as below.
\begin{algorithm}[H]
% \setstretch{1.15}
\begin{algorithmic}[1]
\State \textbf{Input:} Budget $T_1$, reference price $\targetRefPrice$,
price upper bound $\priceUB$.
\State \textbf{Initialization:} Initialize $p_1 = \greedyPrice_1 \in [0, \targetRefPrice]$ arbitrarily; 
parameter $\distance 
\gets 
\frac{1}{2}\left(\targetRefPrice - \max_{\basePara\in\baseParaSpace}\frac{\baseDemandParaB}{2\baseDemandParaA}\right)\wedge
\frac{\priceUB}{2}
$.
\State \textbf{Initialization:} $t\gets 1, s \gets 1$.
\While{$t < T$ or $\learnGRCounter < T_1$}
    \State $t \gets t + \SteerRef(t, \rePrice_t, \targetRefPrice)$.
    \State 
    Pick $\randomDirec\in\{-1, 1\}$ uniformly at random. 
    \Comment{Notice that we now have $\rePrice_t = \targetRefPrice$}
    \State 
    Set the price $p_t$ at time $t$ as
    $\chosenGR_s \gets \greedyPrice_s + \distance \randomDirec$, and observe the realized demand $\demand_{t}(p_t, \targetRefPrice)$.
    \label{line:set price}
    \State 
    Let $\adjustedGrad_{\learnGRCounter} = \frac{\chosenGR_s \demand_{t}(\chosenGR_s; \targetRefPrice)}{\distance}\randomDirec$.
    \State
    Let $\greedyPrice_{\learnGRCounter+1} \gets \Proj_{[\distance, \targetRefPrice - \distance]} \left(\greedyPrice_{\learnGRCounter} + \frac{1}{\learnGRCounter\cdot 2\priceUB}\adjustedGrad_{\learnGRCounter}\right)$.
    \label{line:projection}
    \State 
    $\learnGRCounter \gets \learnGRCounter +1; 
    t \gets t+1$.
\EndWhile
\State \textbf{Return} 
$\estGreedy(\rePrice)  = 
\sfrac{\sum_{s = 1}^{T_1} \greedyPrice_s }{T_1}$, 
and the current time $t$.
\end{algorithmic}
\caption{\learnGR: 
A zeroth-order convex 
optimization for learning greedy price}
\label{algo:zeroth-order arbitrary}
\end{algorithm}


Given a reference price $\rePrice\in[0, \priceUB]$,  we define the following {\em constrained} greedy price, referred to as $\conGreedyPrice(\rePrice)$,  with restricting it to be in the range $[0, \rePrice]$:
\begin{equation}
    \label{eq:constrained greedy price}
    \conGreedyPrice(\rePrice) 
    \triangleq 
    \max_{p\in[0, \rePrice]}~ 
    p \left(\baseDemand(p) 
    + \negativeRef(\rePrice - p) \wedge 0 
    + \positiveRef(\rePrice - p) \vee 0\right)
    = \max_{p\in[0, \rePrice]}~ 
    p \left(\baseDemand(p) 
    + \positiveRef(\rePrice - p)\right)~.
\end{equation}
We now notice the following relation between 
the reference price $\rePrice$ and its corresponding constrained
greedy price $\conGreedyPrice(\rePrice)$:
\begin{lemma}
\label{lem:constrained greedy}
For any reference price $\rePrice\in[\max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA}, \priceUB]$, 
we have $\conGreedyPrice(\rePrice) = \trueCOne\rePrice+\trueCTwo$ and moreover
$\conGreedyPrice(\rePrice) \le \rePrice$.
\end{lemma}
\begin{proof}[Proof of \Cref{lem:constrained greedy}]
By the first-order condition for the 
maximization problem in \eqref{eq:constrained greedy price}, we know that 
\begin{equation*}
    \begin{aligned}
    \conGreedyPrice(\rePrice) 
    & = 
    \left\{\begin{array}{ll}
    \displaystyle \trueCOne\rePrice+\trueCTwo & \text{if } 
    \displaystyle \trueCOne\rePrice+\trueCTwo  \le \rePrice \\
    \rePrice  & \text{if } 
    \displaystyle \trueCOne\rePrice+\trueCTwo > \rePrice
    \end{array}
    \right. 
    \end{aligned}
\end{equation*}
Below we show that when $\rePrice\in[\max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA}, \priceUB]$, we always have 
$\trueCOne\rePrice+\trueCTwo \le \rePrice$. To see this
\begin{align*}
    \rePrice - (\trueCOne\rePrice+\trueCTwo)
    = 
    \frac{\rePrice(2\baseDemandParaA + \positiveRef) - \baseDemandParaB}{2(\baseDemandParaA+\positiveRef)}
    = 
    (2\baseDemandParaA + \positiveRef)\frac{\rePrice - \frac{\baseDemandParaB}{2\baseDemandParaA + \positiveRef}}{2(\baseDemandParaA+\positiveRef)}
    \ge 
    (2\baseDemandParaA + \positiveRef)\frac{\rePrice - \max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA}}{2(\baseDemandParaA+\positiveRef)} \ge 0
\end{align*}
Thus, the proof completes.
\end{proof}



We now show how to use \Cref{algo:equal ref}
with a modified \Cref{algo:zeroth-order} (see below \Cref{algo:zeroth-order arbitrary})
solve the case when $\positiveRef\neq\negativeRef$. 
We define $\Delta \triangleq \priceUB - 
\max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA} > 0$.
In \Cref{algo:equal ref}, we choose 
$\rePrice_a 
= \max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA} + \frac{\Delta}{4}
= 
\frac{\priceUB}{4} + 
\max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{\baseDemandParaA};
% \frac{3\baseDemandParaBUB}{8\baseDemandParaALB}; 
\rePrice_b 
= \max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA} % \frac{\baseDemandParaBUB}{2\baseDemandParaALB} 
+ \frac{\Delta}{2}
= \frac{\priceUB}{2} +\max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{4\baseDemandParaA} % \frac{\baseDemandParaBUB}{4\baseDemandParaALB}
$. 
Notice that with the above choices, 
we have $\rePrice_a, \rePrice_b \in [\max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA}, \priceUB]$. 
Moreover, for $\rePrice\in\{\rePrice_a, \rePrice_b\}$ we have
\begin{align*}
    \rePrice - \conGreedyPrice(\rePrice)
    = 
    (2\baseDemandParaA + \positiveRef)\frac{\rePrice - \frac{\baseDemandParaB}{2\baseDemandParaA + \positiveRef}}{2(\baseDemandParaA+\positiveRef)}
    \ge 
    (2\baseDemandParaA + \positiveRef)\frac{\rePrice - \max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA}}{2(\baseDemandParaA+\positiveRef)}
    % \ge 
    % \left(\rePrice - \frac{\baseDemandParaBUB}{2\baseDemandParaALB}\right) \frac{2\baseDemandParaALB + \maxRef}{2(\baseDemandParaALB + \maxRef)}
    >
    \frac{1}{2}\left(\rePrice - \max_{\basePara\in\baseParaSpace}\sfrac{\baseDemandParaB}{2\baseDemandParaA}\right)~.
\end{align*}
% Similarly, we also have 
% $\rePrice_b - \conGreedyPrice(\rePrice_b)\ge 
% \frac{\Delta}{4} = \frac{1}{2}\left(\rePrice_b - \frac{\baseDemandParaBUB}{2\baseDemandParaALB}\right)$. 
On the other hand, for $\rePrice\in\{\rePrice_a, \rePrice_b\}$, we have
\begin{align*}
    \conGreedyPrice(\rePrice) 
    = 
    \frac{\baseDemandParaB + \positiveRef\rePrice}{2(\baseDemandParaA+\positiveRef)}
    \ge \frac{\priceUB}{2}
    % \ge \frac{\baseDemandParaBLB + \positiveRef\rePrice}{2(\baseDemandParaAUB + \positiveRef)}
    % \ge 
    % \frac{\baseDemandParaBLB}{2\baseDemandParaAUB} 
    % \wedge \frac{\baseDemandParaBLB + \maxRef \rePrice}{2(\baseDemandParaAUB + \maxRef)}~.
\end{align*}
For an input reference price $\targetRefPrice$,
in \Cref{algo:zeroth-order arbitrary},
by setting 
$\distance
\gets 
\frac{1}{2}\left(\targetRefPrice - \max_{\basePara\in\baseParaSpace}\frac{\baseDemandParaB}{2\baseDemandParaA}\right)\wedge
\frac{\priceUB}{2}
% \frac{\baseDemandParaBLB}{2\baseDemandParaAUB} 
% \wedge \frac{\baseDemandParaBLB + \maxRef \targetRefPrice}{2(\baseDemandParaAUB + \maxRef)}
$
and considering the projection function $\Proj_{[\distance, \targetRefPrice - \distance]} (\cdot)$,
we can ensure that the price $p_t$ chosen 
at time $t$ in Line 7 of \Cref{algo:zeroth-order arbitrary} 
must be in the interval $[0, \targetRefPrice]$.\footnote{We note that $[\distance, \targetRefPrice - \distance]$ is a valid price space as we always have $\targetRefPrice > 2\distance$. To see this, notice that we always have $\targetRefPrice
> 2\cdot \frac{1}{2} \left(\targetRefPrice - \max_{\basePara\in\baseParaSpace}\frac{\baseDemandParaB}{2\baseDemandParaA}\right) \ge 2d$.}
This guarantees that the expected demand $\demand(p_t, \targetRefPrice)$ at time $t$ must be 
$\baseDemand(p_t) + \positiveRef(\targetRefPrice - p_t)$.







\begin{proof}[Proof of \Cref{thm:regret upper bound} for arbitrary $\positiveRef, \negativeRef$]
Let $\optPolicy = (p_t^*)_{t\in[T]}$
denotes the optimal pricing policy for the 
reference effects $(\negativeRef, \positiveRef)$, 
and $(\rePrice_t^*)_{t\in[T]}$ is the resulting reference price sequence.
Let $\pricingAlgo$ be the pricing policy implemented by \Cref{algo:equal ref}, and suppose $\exploitT \in [T]$ is the first time round that
the \Cref{algo:equal ref} enters in the Exploitation phase, and let 
$\rePrice_{\exploitT}$ be the corresponding reference price induced by the policy $\pricingAlgo$ at time $\exploitT$.
% Let $\left(p_{t, \rePrice}^*\right)_{t\in[\exploitT, T]}$
% be the optimal pricing policy under the 
% reference price effect $(\negativeRef, \positiveRef)$ 
% over the time window
% $[\exploitT, T]$ with the initial reference $\rePrice$ at time $\exploitT$.
With the above definitions, 
the total regrets of policy $\pi$ can be decomposed as follows: 
\begin{align*}
    & \Reg[\pricingAlgo]{T, \basePara} \\
    =  ~ &  \optVal(\rePrice) - \expect[\policy\sim \pricingAlgo]{\val^{\policy}(\rePrice)} \\
    \le ~ &  \expect[\pricingAlgo]{O\left(\exploitT\revUB\right)+ 
    \optVal(\rePrice_{\exploitT}^*, \exploitT)
    % \Pi\left[[\exploitT, T],  \rePrice_{\exploitT}^*, (p_t^*)_{t\ge \exploitT}\right] 
    - 
    \val^{\approxMD(\priceUB, \exploitT, \paraEst)}(\rePrice_{\exploitT}, \exploitT)} \\
    % \Pi\left[[\exploitT, T],  \rePrice_{\exploitT}, (p_t)_{t\ge \exploitT}\right] \\
    \overset{(a)}{\le} ~ & 
    \expect[\pricingAlgo]{O\left(\exploitT\revUB\right)+ \optVal(\priceUB, \exploitT)
    - \val^{\approxMD(\priceUB, \exploitT, \paraEst)}(\rePrice_{\exploitT}, \exploitT)} \\
    \overset{(b)}{\le}  ~ & 
    \expect[\pricingAlgo]{O\left(\exploitT\revUB\right)+ \optVal(\priceUB, \exploitT)
    - \val^{\approxMD(\priceUB, \exploitT, \paraEst)}(\priceUB, \exploitT)
    + O\left((\positiveRef+\negativeRef)\priceUB(\priceUB - \rePrice_{\exploitT}) \exploitT \ln \frac{T}{\exploitT}\right)}
    % \Pi\left[[\exploitT, T],  \priceUB, (p_t)_{t\ge \exploitT}\right] 
     \\
    \overset{(c)}{\le} ~ & 
    \expect[\pricingAlgo]{O\left(\exploitT\revUB\right)+ 
    O\left(\priceUB^2 \left\|\truePara - \paraEst\right\|^2 (T-\exploitT) \left(\ln \frac{T}{\exploitT}\right)^2\right)
    + O\left((\positiveRef+\negativeRef)\priceUB(\priceUB - \rePrice_{\exploitT}) \exploitT \ln \frac{T}{\exploitT}\right) }
\end{align*}
where 
inequality (a) holds true by \Cref{lem:opt rev diff w.r.t diff ref},
inequality (b) holds true by \Cref{lem:rev gap fixed policy}.
To see inequality (c), notice that by \Cref{lem:lipschitz error in policy space}, 
the optimal price curve that attains nearly optimal value 
$\optVal(\priceUB, \exploitT)$ is the one defined in \Cref{prop:approx markdown structure}, and the price curve $\approxMD(\priceUB, \exploitT, \paraEst)$
is computed with starting reference price $\priceUB$ and estimated policy parameter
$\paraEst$.
Thus, inequality (c) follows by \Cref{lem:lipschitz error in policy space}.
We can then follow the similar analysis in the proof of 
\Cref{thm:regret upper bound} to conclude the desired regrets. 
% let $(\rePrice_{t, \priceUB})_{t\ge \exploitT}$ (resp.\ $(\rePrice_{t, \rePrice_{\exploitT}})_{t\ge \exploitT}$) be the resulting reference price sequence under the policy $(p_t)_{t\ge \exploitT}$
% given the initial reference price to be $\priceUB$ (resp.\ $\rePrice_{\exploitT}$) at time 
% $\exploitT$
% we notice that
% \begin{align*}
%     & \Pi\left[[\exploitT, T],  \priceUB, (p_t)_{t\ge \exploitT}\right] - 
%     \Pi\left[[\exploitT, T],  \rePrice_{\exploitT}, (p_t)_{t\ge \exploitT}\right] \\
%     = ~ &  
%     \sum_{t=\exploitT}^T 
%     p_t \cdot \negativeRef\left((\rePrice_{t, \priceUB} - p_t) \wedge 0 - (\rePrice_{t, \rePrice_{\exploitT}}- p_t)\wedge 0\right)
%     + 
%     p_t \cdot \positiveRef\left((\rePrice_{t, \priceUB} - p_t) \vee 0 - (\rePrice_{t, \rePrice_{\exploitT}}- p_t)\vee 0\right)\\
%     \le ~ &  
%     \sum_{t=\exploitT}^T 
%     p_t \cdot (\positiveRef+\negativeRef) (\rePrice_{t, \priceUB} - \rePrice_{t, \rePrice_{\exploitT}})\\
%     = ~ &  O\left(\priceUB (\positiveRef+\negativeRef) (\priceUB - \rePrice_{\exploitT})\exploitT\ln \frac{T}{\exploitT}\right)
% \end{align*}

% We now proceed to bound the difference $\optVal(\rePrice_{\exploitT}^*, \exploitT)
%     - \val^{(p_t)_{t\ge \exploitT}}(\priceUB, \exploitT)$. 
% Notice that from \Cref{lem:markdown for priceUP as initial}, 
% we know that for any $(\negativeRef, \positiveRef)$, when the initial reference price is $\priceUB$, the optimal price curve 
% $(p_{t, \priceUB}^*)_{t\ge \exploitT}$ is a markdown price curve.
% Moreover, recall that the pricing policy $(p_t)_{t\ge \exploitT}$ is defined as \Cref{defn:policy class}, 
% thus, the policy $(p_t)_{t\ge \exploitT}$ is also markdown pricing policy. 
% Thus, we have 
% \begin{align*}
%     & \Pi\left[[\exploitT, T],  \priceUB, (p_{t, \priceUB}^*)_{t\ge \exploitT}\right] 
%     - \Pi\left[[\exploitT, T],  \priceUB, (p_t)_{t\ge \exploitT}\right] \\
%     \overset{(a)}{=} ~ & 
%     \sum_{t=\exploitT}^T p_{t, \priceUB}^* \baseDemand(p_{t, \priceUB}^*) + \positiveRef p_{t, \priceUB}^*(\rePrice_{t, \priceUB}^* - p_{t, \priceUB}^*)
%     - 
%     \sum_{t=\exploitT}^T p_t \baseDemand(p_t) + \positiveRef p_t(\rePrice_t - p_t) \\
%     \overset{(b)}{=} ~ & 
%     O\left(\priceUB^2 \left\|\truePara - \para\right\|^2 (T-\exploitT) \left(\ln \frac{T}{\exploitT}\right)^2\right)
% \end{align*}
% where equality (a) is due to the fact that 
% $\rePrice_{t, \priceUB}^* \le p_{t, \priceUB}^*$
% and $\rePrice_t \le p_t$ for all $t\ge \exploitT$, 
% and equality (b) is due to \Cref{lem:lipschitz error in policy space}.
% Now following the similar analysis in the proof of \Cref{thm:regret upper bound}, we can conclude the desired regrets. 
\end{proof}








==> algo-design/apx-unbounded-noise.tex <==

\newcommand{\subgauPara}{\tau}

\subsection{Useful High Probability Bounds}

\begin{definition}
\label{defn:subgaussian}
A random variable $X$ is said to be $\subgauPara$-subgaussian if $\expect{\sfrac{X^2}{\subgauPara^2}}\le 2$.
\end{definition}

\begin{lemma}
\label{ineq:subexpon}
Suppose $X_1, \ldots, X_n$ 
are independent and identically
distributed sub-Gaussian random variables with parameter $\sigma$. 
Then each $X_i$ is sub-exponential random variables with parameter
$(4\sqrt{2}\sigma^2, 4\sigma^2)$.
When $t \ge 8\sigma^2$, we have
\begin{align*}
    \prob{\left|\frac{1}{n}\sum_{i=1}^n X_i^2 - \expect{X^2}\right| \ge t} \le 2\exp\left(-\frac{nt}{8\sigma^2}\right)
\end{align*}
\end{lemma}


\subsection{The Estimation Error with Unbounded Demand Shocks}
In this section, we provide the estimation error 
when the noise follows an unbounded sub-Gaussian distribution, namely, the demand shocks $\{\shock_t\}$ are independent and identically distributed variables that are $\sigma$-subgaussian and have zero mean.
The main results in this section are summarized as follows: 
\begin{proposition}
\label{prop:opt greedy est error subgaussian}
Let $\delta < \sfrac{1}{e}$ and 
let $\rePrice\in[0, \priceUB]$ be the reference price to the input of \Cref{algo:zeroth-order}. 
For any $T \ge 4$, we have the following holds with probability at least $1 - \delta$:
\begin{align*}
    \left|p_t - \greedyPrice(\rePrice)\right|
    \le 
    O\left( \frac{(\lipConstEqualRef + \subgauPara)^2 \log \sfrac{1}{\delta}}{\strongConcavPara^2 t} \right)
\end{align*}
where $\subgauPara = \sigma \priceUB \cdot \left((\baseDemandParaA + \eta) \distance 
+ \frac{\priceUB(\distance + \eta \priceUB) + \priceUB^2(\baseDemandParaA+\eta)}{\distance^2}\right)$.
\end{proposition}
We start our analysis from \Cref{lem:error bound via grad diff}. 
Below we show that we can bound 
the summation of the estimated gradients 
$\sum_{i=2}^t\adjustedGrad_i^2$ (see \Cref{lem:bound the sum of adjustedGrad}) and
the summation  
$\sum_{i=2}^t (i-1)\gradientDiff_i(p_i - \greedyPrice(\rePrice))$ (see \Cref{lem:bound the sum of martingale}). 
Then the above results immediately follow
by plugging the results in these two lemmas.
 

\begin{lemma}
\label{lem:subgau gradient diff}
The random variable $\gradientDiff_t$ is $\subgauPara$-subgaussian 
with the zero-mean conditioned on $\filtering_{t-1}$
where $\subgauPara = \sigma \priceUB \cdot \left((\baseDemandParaA + \eta) \distance 
+ \frac{\priceUB(\distance + \eta \priceUB) + \priceUB^2(\baseDemandParaA+\eta)}{\distance^2}\right)$.
\end{lemma}
\begin{proof}
We begin with simplifying the expression of variable $\gradientDiff_t$.
\begin{align*}
    \gradientDiff_t
    & = \adjustedGrad_t - \gradient_t \\
    & = \frac{\chosenPrice_t \demand_t(\chosenPrice_t; \rePrice)}{\distance}\randomDirec -  \frac{\partial\staticRev{p_t;\rePrice}}{\partial p_t}\\
    & = 
    \frac{\randomDirec}{\distance} \cdot \left(- (\baseDemandParaA + \eta)\chosenPrice_t^2 + (\baseDemandParaB-\eta\rePrice)\chosenPrice + \shock_t\chosenPrice_t\right) - \left(-2(\baseDemandParaA+\eta)p_t + \baseDemandParaB - \eta\rePrice\right)\\
    & = 
    \frac{\randomDirec}{\distance} \cdot \left(- (\baseDemandParaA + \eta)\left(p_t + \distance\randomDirec\right)^2 + (\baseDemandParaB-\eta\rePrice)\left(p_t + \distance\randomDirec\right) + \shock_t\left(p_t + \distance\randomDirec\right)\right) -  \left(-2(\baseDemandParaA+\eta)p_t + \baseDemandParaB - \eta\rePrice\right)\\
    & = 
    \frac{1}{\distance} \left(-(\baseDemandParaA + \eta)\distance^2 \randomDirec^3 
    + 
    \left(-(\baseDemandParaA + \eta)p_t^2 + p_t(\distance -\eta\rePrice) + \shock_tp_t\right)\randomDirec\right)
    + 
    \left(-2(\baseDemandParaA+\eta)p_t + \baseDemandParaB - \eta\rePrice \right)\randomDirec^2
    + \shock_t\randomDirec^2 \\
    & \quad -  \left(-2(\baseDemandParaA+\eta)p_t + \baseDemandParaB - \eta\rePrice\right)\\
    & = \frac{1}{\distance} \left(-(\baseDemandParaA + \eta)\distance^2 \randomDirec^3 
    + 
    \left(-(\baseDemandParaA + \eta)p_t^2 + p_t(\distance -\eta\rePrice) + \shock_tp_t\right)\randomDirec\right) + \shock_t \\
    & = 
    \frac{1}{\distance} \left(
    (-(\baseDemandParaA + \eta)\distance^2 \randomDirec^2 -(\baseDemandParaA + \eta)p_t^2 + p_t(\distance -\eta\rePrice))\randomDirec
    + 
    \shock_tp_t\randomDirec\right) + \shock_t \\
    & = c_{1, t} \randomDirec + c_{2, t} \randomDirec \shock_t + \shock_t
\end{align*}
where $c_{1, t} \triangleq \frac{1}{\distance} 
\left(-(\baseDemandParaA + \eta)\distance^2 -(\baseDemandParaA + \eta)p_t^2 + p_t(\distance -\eta\rePrice)\right)$ and $c_{2, t} \triangleq  \frac{p_t}{\distance}$.
For any $\lambda \in \R$, consider 
\begin{align*}
    \expect{\exp(\lambda \gradientDiff_t) \mid \filtering_{t-1}}
    & = \expect{\exp(\lambda(c_{1, t} \randomDirec + c_{2, t} \randomDirec \shock_t + \shock_t)) \mid \filtering_{t-1}} \\
    & = \frac{1}{2} \left(\expect{\exp(\lambda(c_{1, t} + c_{2, t} \shock_t + \shock_t)) \mid \filtering_{t-1}} 
    +  \expect{\exp(-\lambda(c_{1, t} - c_{2, t} \shock_t + \shock_t)) \mid \filtering_{t-1}} \right)
\end{align*}
Notice that 
\begin{align*}
    \expect{\exp(\lambda(c_{1, t} + c_{2, t} \shock_t + \shock_t)) \mid \filtering_{t-1}}
    & = \exp(\lambda c_{1, t}) \expect{\exp(\shock_t\lambda(1 + c_{2, t})) \mid \filtering_{t-1}} \\
    & \le \exp(\lambda c_{1, t})\exp\left(\frac{\sigma^2 (1+c_{2, t})^2 \lambda^2}{2}\right)\\
    \expect{\exp(\lambda(-c_{1, t} - c_{2, t} \shock_t + \shock_t)) \mid \filtering_{t-1}}
    & \le  
    \exp(-\lambda c_{1, t})\exp\left(\frac{\sigma^2 (1 - c_{2, t})^2 \lambda^2}{2}\right)
\end{align*}
Thus, we have
\begin{align}
    \expect{\exp(\lambda \gradientDiff_t) \mid \filtering_{t-1}}
    \le \frac{1}{2}\left(
    \exp(\lambda c_{1, t})\exp\left(\frac{\sigma^2 (1+c_{2, t})^2 \lambda^2}{2}\right)
    + \exp(-\lambda c_{1, t})\exp\left(\frac{\sigma^2 (1 - c_{2, t})^2 \lambda^2}{2}\right)
    \right)
    \label{lemA1:helper}
\end{align}
Recall that in \Cref{algo:zeroth-order}, we have $p_t \in [\distance, \priceUB-\distance]$, thus, $(1-c_{2, t})^2 \le (1+c_{2, t})^2 \le \frac{\priceUB^2}{\distance^2}$. 
Back to \eqref{lemA1:helper}, we have
\begin{align*}
    \expect{\exp(\lambda \gradientDiff_t) \mid \filtering_{t-1}}
    & \le 
    \exp\left(\frac{\sigma^2\lambda^2 (\sfrac{\priceUB}{\distance})^2}{2}\right) \cdot\frac{1}{2}\left(\exp(\lambda c_{1, t}) + \exp(-\lambda c_{1, t})\right)\\
    & \le 
    \exp\left(\frac{\sigma^2\lambda^2 (\sfrac{\priceUB}{\distance})^2}{2}\right) \cdot\frac{1}{2}\left(\sum_{k=0}^{\infty} \frac{(\lambda c_{1, t})^k}{k!} + \sum_{k=0}^{\infty} \frac{(-\lambda c_{1, t})^k}{k!}\right)\\
    & \le 
    \exp\left(\frac{\sigma^2\lambda^2 (\sfrac{\priceUB}{\distance})^2}{2}\right)
    \exp\left(\frac{c_{1, t}^2\lambda^2}{2}\right) \\
    & = \exp\left(\frac{\sigma^2 (\sfrac{\priceUB}{\distance})^2 \bar{c}^2}{2}\lambda^2\right)
\end{align*}
where we always have $|c_{1, t}| 
\le \bar{c} \triangleq (\baseDemandParaA + \eta) \distance 
+ \frac{\priceUB(\distance + \eta \priceUB) + \priceUB^2(\baseDemandParaA+\eta)}{\distance}$.
\end{proof}


\begin{lemma}
\label{lem:bound the sum of adjustedGrad}
For any $\delta \in (0, 1)$, 
we have the following holds with probability 
at least $1 - \delta$:
\begin{align*}
    \sum_{i=2}^t \adjustedGrad_i^2 
    \le 
    \frac{\priceUB^2}{\distance^2}
    \left(t(\baseDemandParaBUB + \maxRef\priceUB)^2 + t\sigma^2 + 8\sigma^2 \log \frac{1}{\delta}\right)
\end{align*}
\end{lemma}
\begin{proof}
By definition, we have
\begin{align*}
    \sum_{i=2}^t \adjustedGrad_i^2
    =     
    \sum_{i=2}^t \frac{\randomDirec^2}{\distance^2}\left(\chosenPrice_i(\demand(\chosenPrice_i;\rePrice) + \shock_i)\right)^2
    & = 
    \sum_{i=2}^t
    \frac{1}{\distance^2}\left(\chosenPrice_i(\demand(\chosenPrice_i;\rePrice) + \shock_i)\right)^2 \\
    & \le 
    \sum_{i=2}^t
    \frac{2}{\distance^2}\left(\chosenPrice_i^2\demand(\chosenPrice_i; \rePrice)^2 + \chosenPrice_i^2\shock_i^2\right)\\
    & \le
    \frac{2t}{\distance^2}
    \priceUB^2(\baseDemandParaBUB + \maxRef\priceUB)^2
    + 
    \frac{2\priceUB^2}{\distance^2}\sum_{i=2}^t\shock_i^2
\end{align*}
Recall that $\{\shock_i\}$ are independent 
sub-Gaussian random variables with the parameter $\sigma$. 
Thus, with \Cref{ineq:subexpon}, we know that $\{\shock_i^2\}$ are 
are sub-exponential random variables with parameter
$(4\sqrt{2}\sigma^2, 4\sigma^2)$.
Consequently, we have
the following holds with probability at least $1 - \delta$:
\begin{align*}
    \left|\frac{1}{t-1}\sum_{i=2}^t \shock_i^2 - \sigma^2\right| \le \frac{8\sigma^2}{t-1} \log \frac{1}{\delta}
\end{align*}
which implies that 
$\frac{1}{t-1}\sum_{i=2}^t \shock_i^2\le (t-1)\sigma^2 + 8\sigma^2 \log \sfrac{1}{\delta}$ holds with probability at least $1-\delta$.
\end{proof}

\begin{lemma}
\label{lem:bound the sum of martingale}
For any $\delta \in (0, 1)$, 
we have the following holds with probability 
at least $1 - \delta$:
\begin{align*}
    \sum_{i=2}^t (i-1)\gradientDiff_i(p_i - \greedyPrice(\rePrice)) 
    \le O\left(\frac{t (\lipConstEqualRef+\subgauPara)^2}{\strongConcavPara} \log \frac{1}{\delta}\right)
\end{align*}
where $\subgauPara$ is defined as in \Cref{lem:subgau gradient diff}.
\end{lemma}
\begin{proof}
For notation simplicity, 
define $z_t \triangleq (t-1)\gradientDiff_t(p_t - \greedyPrice(\rePrice))$.
We also define 
$v_{t-1} \triangleq 2\subgauPara^2(t-1)^2(p_t - \greedyPrice(\rePrice))^2$, and 
$V_{t-1} \triangleq \sum_{s=1}^{t} v_{s-1}$. 
We note that  $v_{t-1}$ is 
$\filtering_{t-1}$-measurable.
Recall that in \Cref{lem:subgau gradient diff}, we 
have shown the variable $\gradientDiff_t$ is $\subgauPara$-subgaussian, thus we have 
for any $\lambda \in \R$.
\begin{align}
    \label{ineq:subgaussian on v}
    \expect{\exp(\lambda z_t) \mid \filtering_{t-1}}
    = \expect{\exp(\lambda (t-1)\gradientDiff_t(p_t - \greedyPrice(\rePrice))) \mid \filtering_{t-1}}
    \overset{(a)}{\le}
    \exp\left(\frac{\lambda^2}{2} v_{t-1}\right)~.
\end{align}
where inequality (a) is due to \Cref{defn:subgaussian}. 

To finish the proof, we use the following two 
technique lemmas:
\begin{lemma}[\citealp{HLR-19b}, Lemma C.11]
\label{lem:margingale helper1}
There exists non-negative constants $(\alpha_i)_{i\in[t]}$ where each $\alpha_i = O\left((\lipConstEqualRef+\subgauPara)^2\frac{i}{\strongConcavPara}\right)$
and $\beta = O\left(\frac{(\lipConstEqualRef+\subgauPara)^4}{\strongConcavPara^2}t^2\right)$ such that for every $\delta\in(0, 1)$,
we have $V_t \le \sum_{i=1}^t \alpha_i z_i + \beta \log \frac{1}{\delta}$ with probability at least $1 - \delta$.
\end{lemma}

\begin{lemma}[\citealp{HLR-19a}, Theorem 3.3]
\label{lem:margingale helper2}
Let $\{z_t, \filtering_t\}_{t\ge 1}$ be a martingale difference sequence.
Suppose that, for any $t \ge 1$, 
$v_{t-1}$ are non-negative $\filtering_{t-1}$-measurable random variables satisfying  
$\expect{\exp(\lambda z_t) \mid \filtering_{t-1}}
\le
\exp\left(\frac{\lambda^2}{2} v_{t-1}\right)$ for all $\lambda > 0$. 
Let $Z_t = \sum_{s=1}^t z_s$ and $V_t = \sum_{s=1}^t v_{s-1}$. 
Then we have
Suppose there exists $(\alpha_i)_{i\in[t]}, \beta \in \R_{\ge 0}$ 
such that for every $\delta\in(0, 1)$,
$V_t \le \sum_{i=1}^t \alpha_i z_i + \beta \log \frac{1}{\delta}$.
Let $\bar{\alpha} = \max_{t\ge 1} \alpha_t$, we then have
\begin{align*}
    \prob{Z_t \ge Z}  \le 
    \exp\left( - \frac{Z^2}{4\bar{\alpha} Z + 8\beta}\right) + \delta
\end{align*}
\end{lemma}
From \eqref{ineq:subgaussian on v}, we know that
$\expect{\exp(\lambda z_t) \mid \filtering_{t-1}} \le 
\exp\left(\sfrac{\lambda^2 v_{t-1}}{2}\right)$
for all $\lambda > 0$. 
Thus, with \Cref{lem:margingale helper1}, 
we have that for every $\delta \in (0, 1)$,
$V_t \le  \sum_{i=1}^t \alpha_i z_i + \beta \log \frac{1}{\delta}$ holds  with probability at least $1-\delta$.
With $\bar{\alpha} \gets O\left(\frac{t(\lipConstEqualRef + \subgauPara)^2}{\strongConcavPara}\right)$ and 
$\beta \gets \left(\bar{\alpha}^2\log \frac{1}{\delta}\right)$ in \Cref{lem:margingale helper2}, 
and $Z \gets O\left(\bar{\alpha} \log \frac{1}{\delta}\right)$,
we can finish the proof.
\end{proof}







==> learning_via_greedy.tex <==






% \begin{algorithm2e}
% \setstretch{1.25}
% \caption{Optimal learning from greedy}
% \label{algo:learn from greedy}
% \SetAlgoLined\DontPrintSemicolon
% \textbf{Input:} Horizon $T$. \\ 
% \textbf{Initialize:} $T_1 \gets $ \\
% \end{algorithm2e}





\begin{algorithm}
\setstretch{1.15}
\begin{algorithmic}[1]
\State \textbf{Input:} Time horizon $T$, initial reference price $\rePrice_t$. 
\State \textbf{Initialization:} $T_1\gets $; 
$\rePrice_a \gets \rePrice_1$, and $\rePrice_b \gets \sfrac{\rePrice_1}{2}$.\\
\Comment{Exploration phase 1:\ learning an estimate $\estGreedy(\rePrice_a)$ of  
$\greedyPrice(\rePrice_a)$ for reference price $\rePrice_a$}\\
\Comment{Smoothing phase:\ smooth the current reference price to be $\rePrice_b$}\\
\Comment{Exploration phase 2:\ learning an estimate $\estGreedy(\rePrice_b)$ of  
$\greedyPrice(\rePrice_b)$ for reference price $\rePrice_b$}\\
\Comment{Exploitation phase:\ }
\State Compute an estimate of the policy parameter 
$\paraEst = (\estCOne, \estCTwo)$ from \eqref{eq:policy para from greedy}. 
\State Implement the pricing policy $\paraEst = (\estCOne, \estCTwo)$ (see \Cref{defn:policy}) for the remaining rounds. 
\end{algorithmic}
\caption{Learning dynamic pricing policy 
from greedy}
\label{algo:learn from greedy}
\end{algorithm}


\begin{algorithm}
\setstretch{1.15}
\begin{algorithmic}[1]
\State \textbf{Input:} Time horizon $T$, reference price $\rePrice$,
strong concavity parameter $\stronglyCovxPara > 0$, and the 
distance parameter $\distance\in (0, 1]$.
\State \textbf{Initialization:} Initialize $p_1 \in \priceSpace$ arbitrarily.
\While{$t < T$}
    \State Pick $\randomDirec\in\{-1, 1\}$ uniformly at random
    \State Choose the price $p_t \gets p_t + \distance \randomDirec$, and observe the realized demand $\demand_t(p_t)$
    \State 
    Let $\gradient_t = \frac{p_t \demand_t(p_t)}{d}\randomDirec$
    \State
    Let $p_{t+1} \gets \Proj_{\priceSpace} \left(p_t - \frac{1}{\stronglyCovxPara t}\gradient_t\right)$
\EndWhile
\end{algorithmic}
\caption{Learning greedy price}
\label{algo:zeroth-order}
\end{algorithm}

Fix a reference price $\rePrice\in\priceSpace$, 
define the following single-round expected revenue function:
\begin{align*}
    \Pi[\rePrice, p] = p\cdot \left(\baseDemandParaB - \baseDemandParaA p + \eta (\rePrice - p)\right)
\end{align*}

\begin{lemma}[Single-ground greedy pricing policy]
Fix a time $t_1$ and its reference price $\rePrice_{t_1}=\rePrice$, then the greedy price that maximizes the revenue of this time round is
\begin{align*}
    \greedyPrice(\rePrice) = \trueCOne \rePrice + \trueCTwo \in \argmax_{p\in\priceSpace }\Pi[\rePrice, p]
\end{align*}
Moreover, function $\Pi[\rePrice, p]$ is $2(\baseDemandParaA+\eta)$-strongly concave. 
\end{lemma}



Given two difference reference prices $\rePrice_a, \rePrice_b$, 
and given the greedy prices $\greedyPrice(\rePrice_a), \greedyPrice(\rePrice_b)$
for these two reference prices, respectively, we have
\begin{align}
    \trueCOne = \frac{\greedyPrice(\rePrice_b) - \greedyPrice(\rePrice_a)}{\rePrice_b-\rePrice_a};
    \quad 
    \trueCTwo = \greedyPrice(\rePrice_a) - \trueCOne \rePrice_a = 
    \frac{\greedyPrice(\rePrice_a)\rePrice_b - \greedyPrice(\rePrice_b)\rePrice_a}{\rePrice_b-\rePrice_a}
\end{align}
Given an estimate $\estGreedy(\rePrice_a)$ to 
the price $\greedyPrice(\rePrice_a)$, and an estimate 
$\estGreedy(\rePrice_b)$ to 
the price $\greedyPrice(\rePrice_b)$, we can compute 
an estimate $\paraEst= (\estCOne, \estCTwo)$ to the 
$\truePara = (\trueCOne, \trueCTwo)$ as follows
\begin{align}
    \label{eq:policy para from greedy}
    \estCOne = \frac{\estGreedy(\rePrice_b) - \estGreedy(\rePrice_a)}{\rePrice_b-\rePrice_a};
    \quad 
    \estCTwo =  
    \frac{\estGreedy(\rePrice_a)\rePrice_b - \estGreedy(\rePrice_b)\rePrice_a}{\rePrice_b-\rePrice_a}
\end{align}

\begin{lemma}
We have the following guarantees for the estimated 
prices $\estGreedy(\rePrice_a), \estGreedy(\rePrice_b)$:
\begin{align*}
    \prob{\left|\estGreedy(\rePrice_a) - \greedyPrice(\rePrice_a)\right| \ge \frac{\log \frac{\log T_1}{\delta}}{T_1}}
    \le \delta; \quad
    \prob{\left|\estGreedy(\rePrice_b) - \greedyPrice(\rePrice_b)\right| \ge \frac{\log \frac{\log T_1}{\delta}}{T_1}}
    \le \delta
\end{align*}
\end{lemma}

\begin{lemma}
Fix a time window $[t_1,t_2]$, an initial reference price $\rePrice_{t_1} = \rePrice$ at time $t_1$. 
Given a pricing policy $\para = (p_{t_1}(y, z), y, z)$,
we define following cumulative revenue function 
for this time window $[t_1,t_2]$:
\begin{align*}
    \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]
    = \sum_{t=t_1}^{t_2} p_t(y, z)(\baseDemandParaB -\baseDemandParaA p_t(y, z))
    + \eta p_t(y, z)(\rePrice_t(y, z) - p_t(y, z))
\end{align*}
where $(p_t(y, z))_{t\in[t_1,t_2]}$ is defined as in \Cref{defn:pricing policy}
with policy $\para = (p_{t_1}(y, z), y, z)$
and the initial price $p_{t_1}(y, z)$ is computed as in \Cref{lem:initial price characterization}. 
Then we have
\begin{align*}
    \trueCOne, \trueCTwo \in \argmax_{y, z} \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]
\end{align*}
and moreover, we have 
\begin{align*}
    \Pi[[t_1,t_2], \rePrice, (p_{t_1}(\trueCOne, \trueCTwo), \trueCOne, \trueCTwo)]
    -
    \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)] 
    \le O\left(\left(|\trueCOne-y|^2\vee |\trueCTwo-z|^2\right)(t_2-t_1)\ln t_2\right)
\end{align*}
\end{lemma}
\begin{proof}
Recall that we can write the revenue function 
$\Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]$ as follows
\begin{align*}
    \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]
    & = 
    \sum_{t=t_1}^{t_2}
    p_t(y, z)(\baseDemandParaB - \baseDemandParaA p_t(y, z))
    + \eta p_t(y, z)(\rePrice_t(y, z) - p_t(y, z)) + \eta p_t(y, z) \cdot \sum_{s=t+1}^{t_2}\frac{p_s(y, z)}{s} \\
    & = 
    \sum_{t=t_1}^{t_2}
    p_t(y, z)\left(\baseDemandParaB - (\baseDemandParaA + \eta) p_t(y, z) + \eta \left(
    \rePrice_t(y, z) + \sum_{s=t+1}^{t_2}\frac{p_s(y, z)}{s}
    \right)\right)\\
    & =
    2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2}
    p_t(y, z)\left(\trueCTwo - \frac{1}{2} p_t(y, z) + \trueCOne \left(
    \rePrice_t(y, z) + \sum_{s=t+1}^{t_2}\frac{p_s(y, z)}{s}
    \right)\right) \\
    & = 2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2}
    p_t(y, z)\left(\trueCTwo - \frac{1}{2} p_t(y, z) + \trueCOne S_t(y, z)\right)
\end{align*}
where $S_t(y, z) 
\triangleq \rePrice_t(y, z) + \sum_{s=t+1}^{t_2}\frac{p_s(y, z)}{s}
= \frac{t_1 \rePrice + \sum_{s=t_1}^{t-1}p_s(y, z)}{t} + \sum_{s=t+1}^{t_2}\frac{p_s(y, z)}{s}$.
Notice that 
at each round $t\in[t_1, t_2]$, 
when fixing $S_t(y, z) \equiv S_t$, 
by first-order condition,
the optimal price for this current time round is
\begin{align*}
    p_t^* = \trueCTwo + \trueCOne S_t.
\end{align*}
On the other hand, 
under the pricing policy $\para$, we have
\begin{align*}
    p_t(y, z) 
    & = z + y \rePrice_t(y, z) + y \sum_{s=t+1}^{t_2}\frac{p_s(y, z)}{s}
    = z + y\cdot S_t(y, z), \quad \forall t\in[t_1:t_2-1] \\
    p_{t_2}(y, z) 
    & = y \cdot \frac{t_1\rePrice + \sum_{s=t_1}^{t_2-1}p_s(y, z)}{t_2} + z
    = y \cdot S_{t_2}(y, z) + z
\end{align*}
Thus, we know that 
$\trueCOne, \trueCTwo \in \argmax_{y, z} 
\Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]$.

With the definition of $p_t(y, z)$, we have
\begin{align*}
    \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]
    & = 2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2}
    \left(z + y S_t(y, z)\right)
    \left(\trueCTwo - \frac{z}{2} + \left(\trueCOne - \frac{y}{2}\right) S_t(y, z)\right)
\end{align*}
For any $S_t$, we have
\begin{align*}
    \frac{\partial \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial y}
    & = 
    2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2} S_t\left(\trueCTwo - z + S_t \cdot \left(\trueCOne - y\right)\right)\\
    \frac{\partial \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial z}
    & =
    2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2} \left(\trueCTwo - z + S_t \cdot \left(\trueCOne - y\right)\right)
\end{align*}
Notice that 
\begin{align*}
    & 2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2} S_t\left(\trueCTwo - z + S_t \cdot \left(\trueCOne - y\right)\right) \\
    \le ~ &  2(\baseDemandParaA + \eta) 
    \sum_{t=t_1}^{t_2} S_t \left(\estCTwoErr + S_t \estCOneErr\right) \\
    % \le ~ & 
    % 2(\baseDemandParaA + \eta) 
    % \sum_{t=t_1}^{t_2} \left(
    % \frac{t_1 \rePrice + \sum_{s=t_1}^{t-1}\priceUB}{t} + \sum_{s=t+1}^{t_2}\frac{\priceUB}{s}
    % \right) \left(\estCTwoErr + \left(
    % \frac{t_1 \rePrice + \sum_{s=t_1}^{t-1}\priceUB}{t} + \sum_{s=t+1}^{t_2}\frac{\priceUB}{s}
    % \right) \estCOneErr\right) \\
    \le ~ & 
    2(\baseDemandParaA + \eta)  
    \sum_{t=t_1}^{t_2} \estCTwoErr \left(\frac{t_1\rePrice}{t} + \frac{(t-t_1)\priceUB}{t} + \priceUB \ln \frac{t_2}{t}\right)
    + \estCOneErr 
    \left(\frac{t_1\rePrice}{t} + \frac{(t-t_1)\priceUB}{t} + \priceUB \ln \frac{t_2}{t}\right)^2  \\
    \le ~ & 
    2(\baseDemandParaA + \eta)  
    \estCTwoErr\left(t_1\rePrice\ln\frac{t_2}{t_1} + (t_2-t_1)\priceUB - t_1\priceUB \ln \frac{t_2}{t_1} + \priceUB \left((t_2-t_1)\ln t_2 -t_2\ln t_2 + t_2 + t_1\ln t_1-t_1 \right) \right) \\
    &  +
    2(\baseDemandParaA + \eta) \sum_{t=t_1}^{t_2} \estCOneErr 
    \left(\frac{t_1\rePrice}{t} + \frac{(t-t_1)\priceUB}{t} + \priceUB \ln \frac{t_2}{t}\right)^2 \\
    \le ~ & 
    2(\baseDemandParaA + \eta)  
    \estCTwoErr\left(\priceUB(t_2-t_1) - t_1 (2\priceUB - \rePrice) \ln \frac{t_2}{t_1}\right) 
    +
    2(\baseDemandParaA + \eta) \sum_{t=t_1}^{t_2} \estCOneErr 
    \priceUB^2 \left(1 - \frac{t_1}{t}\frac{\priceUB-\rePrice}{\priceUB} +  \ln \frac{t_2}{t}\right)^2 \\
    = ~ & 
    2(\baseDemandParaA + \eta)  
    \estCTwoErr\left(\priceUB(t_2-t_1) - t_1 (2\priceUB - \rePrice) \ln \frac{t_2}{t_1}\right) \\
    & +
    2(\baseDemandParaA + \eta) \sum_{t=t_1}^{t_2} \estCOneErr\priceUB^2  
    \left(\left(1 - \frac{t_1}{t}\frac{\priceUB-\rePrice}{\priceUB}\right)^2 + 2\left(1 - \frac{t_1}{t}\frac{\priceUB-\rePrice}{\priceUB}\right) \ln \frac{t_2}{t}
    + \left(\ln \frac{t_2}{t}\right)^2\right)\\
    \le ~ & 
    2(\baseDemandParaA + \eta)  
    O\left(\estCTwoErr(t_2-t_1)  + \estCOneErr (t_2-t_1)\ln t_2\right)
\end{align*}
Similarly, we have
\begin{align*}
    2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2} \left(\trueCTwo - z + S_t \cdot \left(\trueCOne - y\right)\right)
    \le 
    2(\baseDemandParaA + \eta)  
    O\left(\estCTwoErr(t_2-t_1)  + \estCOneErr (t_2-t_1)\right)
\end{align*}
Thus, we have
\begin{align*}
    \left\|\nabla \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)] \right\|
    \le 
    O\left(\estCTwoErr(t_2-t_1)  + \estCOneErr (t_2-t_1) \ln t_2\right)
\end{align*}
\wtr{
For the second-order derivatives, we have
\begin{align*}
    \frac{\partial^2 \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial y^2}
    & =
    - 2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2} S_t^2 \\
    \frac{\partial^2 \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial z^2}
    & =
    - 2(\baseDemandParaA + \eta)(t_2-t_1)\\
    \frac{\partial^2 \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial y\partial z}
    & =
    - 2(\baseDemandParaA + \eta)\sum_{t=t_1}^{t_2} S_t
\end{align*}
As we can see
\begin{align*}
    \frac{\partial^2 \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial y^2}
    + \frac{\partial^2 \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]}{\partial z^2}
    < 0
\end{align*}
and 
\begin{align*}
    \left(- 2(\baseDemandParaA + \eta)\sum_{t=t_1}^{t_2} S_t\right)^2 - 
    2(\baseDemandParaA + \eta)
    \sum_{t=t_1}^{t_2} S_t^2 \cdot 2(\baseDemandParaA + \eta)(t_2-t_1)
    & =4(\baseDemandParaA+\eta)^2 \left(\left(\sum_{t=t_1}^{t_2} S_t\right)^2 
    - (t_2-t_1) \sum_{t=t_1}^{t_2} S_t^2\right)\\
    & < 0
\end{align*}
where the last inequality is due to 
the Cauchy–Schwarz inequality. 
Thus, function 
$\Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)]$ is concave over the parameter space $(y, z)$. 
Thus, we have
\begin{align*}
    & \Pi[[t_1,t_2], \rePrice, (p_{t_1}(\trueCOne, \trueCTwo), \trueCOne, \trueCTwo)]
    -
    \Pi[[t_1,t_2], \rePrice, (p_{t_1}(y, z), y, z)] \\
    \le ~ & \nabla \Pi[[t_1,t_2], \rePrice,  (p_{t_1}(y, z), y, z)]^\top (\trueCOne - y, \trueCTwo-z)\\
    = ~ & 
    2(\baseDemandParaA + \eta)\left(
    \sum_{t=t_1}^{t_2} S_t\left(\trueCTwo - z + S_t \cdot \left(\trueCOne - y\right)\right), 
    \sum_{t=t_1}^{t_2} \left(\trueCTwo - z + S_t \cdot \left(\trueCOne - y\right)\right)
    \right)^\top (\trueCOne - y, \trueCTwo-z) \\
    \le ~ & 
    2(\baseDemandParaA + \eta)\left(
    \sum_{t=t_1}^{t_2} S_t\left(\estCTwoErr + S_t \cdot \estCOneErr \right), 
    \sum_{t=t_1}^{t_2} \left(\estCTwoErr + S_t \cdot \estCOneErr\right)
    \right)^\top (\estCOneErr, \estCTwoErr)\\
    \le ~ &  2(\baseDemandParaA + \eta)O\left(\max\{\estCOneErr, \estCTwoErr\}^2(t_2-t_1)\ln t_2\right)
\end{align*}
}
\end{proof}

\begin{theorem}
\Cref{algo:learn from greedy} has expected regret as 
$O(\sqrt{T\ln T})$.
\end{theorem}
\begin{proof}
The total regrets can be decomposed as follows: 
\begin{align*}
    \Reg{T} 
    & = O(T_1) + 
    O\left(\frac{1}{\sqrt{T_1}} (T-T_1) \ln T\right) \cdot O\left(\frac{1}{\sqrt{T_1}}\right) \\
    & = O\left(\sqrt{T\ln T}\right)
\end{align*}
\end{proof}


\subsection{Setting with $\negativeRef \neq \positiveRef$}



==> macro.tex <==
\usepackage{amsthm, mathtools, bm, amsmath}
\usepackage{footmisc}
\usepackage[normalem]{ulem}
% \PassOptionsToPackage{numbers, compress}{natbib}
% \usepackage{tcolorbox}
\usepackage{xcolor}
\usepackage{thm-restate}
\usepackage{natbib}
\bibliographystyle{plainnat}
\bibpunct{(}{)}{;}{a}{,}{,}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage[colorlinks=true, linkcolor=blue!70!black, citecolor=blue!70!black,urlcolor=black,breaklinks=true]{hyperref}
\usepackage{comment}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{float}
\usepackage{xspace}
\usepackage{xfrac}
\usepackage{enumitem}
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage[boxed,ruled,algo2e,linesnumbered,noend]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{algorithm}

\usepackage{setspace}
\newcommand{\algcomment}[1]{\textcolor{blue}{\footnotesize{\texttt{\textbf{#1}}}}}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
% \SetCommentSty{mycommfont}
\usepackage{cleveref}




\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}% reset theorem numbering for each chapter

\theoremstyle{plain}
\newtheorem{definition}{Definition}[section] % definition numbers are dependent on theorem numbers
\newtheorem{example}[definition]{Example}
% \newtheorem{assumption}[definition]{Assumption} 
\newtheorem{remark}[definition]{Remark} 
\newtheorem{conjecture}[definition]{Conjecture} 
\newtheorem{task}[definition]{Task} 

\theoremstyle{plain}

\newenvironment{numbereddefinition}[1]{%
\renewcommand{\thedefinition}{#1}%
\begin{definition}}{\end{definition}\addtocounter{definition}{-1}}


\newtheorem{assumption}{Assumption}
% \newtheorem{assumption}[definition]{Assumption} 


\newenvironment{numberedassumption}[1]{%
\renewcommand{\thedefinition}{#1}%
\begin{assumption}}{\end{assumption}\addtocounter{definition}{-1}}



\newcounter{relctr} %% <- counter for relations
\everydisplay\expandafter{\the\everydisplay\setcounter{relctr}{0}} %% <- reset every eq
\renewcommand*\therelctr{\alph{relctr}} %% <- label format
\newcommand\labelrel[2]{%
  \begingroup
    \refstepcounter{relctr}%
    \stackrel{\textnormal{(\alph{relctr})}}{\mathstrut{#1}}%
    \originallabel{#2}%
  \endgroup
}
\AtBeginDocument{\let\originallabel\label} %% <- store original definition


\newcommand{\introthmname}{}
\newtheorem{introthminn}{\introthmname}
\newenvironment{introthm}[1]
  {\renewcommand{\introthmname}{#1}\begin{introthminn}}
  {\end{introthminn}}

\swapnumbers


\newcommand{\squishlist}{
\begin{list}{{{\small{$\bullet$}}}}
{\setlength{\itemsep}{3pt}      \setlength{\parsep}{1pt}
\setlength{\topsep}{1pt}       \setlength{\partopsep}{0pt}
\setlength{\leftmargin}{1em} \setlength{\labelwidth}{1em}
\setlength{\labelsep}{0.5em} } }
\newcommand{\squishend}{  \end{list}}

\newcommand{\Reg}[2][]{\text{\bf REG}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}


\newcommand{\supp}{\cc{supp}}

\newcommand{\rePriceDemand}{R}
\newcommand{\rePrice}{r}
\newcommand{\expRev}{\pi}
\newcommand{\groupNum}{N}
\newcommand{\OPT}{\cc{OPT}}

\newcommand{\priceSpace}{\mathcal{X}}
\newcommand{\priceBudget}{B}

% \newcommand{\valFunc}[2][]{\Pi\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

\newcommand{\baseDemandPara}{b}
\newcommand{\baseDemandParaB}{\baseDemandPara}
\newcommand{\baseDemandParaA}{a}

\newcommand{\priceLB}{\underline{p}}
\newcommand{\priceUB}{\bar{p}}


% Algo design
\newcommand{\staticRev}[2][]{\cc{Rev}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left({\def\givenn{\middle|}#2}\right)}
\newcommand{\realizedDemand}{D}
\newcommand{\para}{\theta}
\newcommand{\truePara}{\para^*}
\newcommand{\paraEst}{\widehat{\para}}
\newcommand{\paraSpace}{\Theta}
\newcommand{\interval}{\mathcal{I}}

\newcommand{\epochLen}{\ell}
\newcommand{\epoch}{\mathcal{E}}
\newcommand{\stageLen}{s}

\newcommand{\trueCOne}{C_1^*}
\newcommand{\trueCTwo}{C_2^*}
\newcommand{\estCOne}{\widehat{C}_1}
\newcommand{\estCTwo}{\widehat{C}_2}
\newcommand{\estInitialP}{\widehat{p}}

\newcommand{\estInitialPErr}{\varepsilon_0}
\newcommand{\estCOneErr}{\varepsilon_1}
\newcommand{\estCTwoErr}{\varepsilon_2}

\newcommand{\estRef}{\widehat{\rePrice}}





